Regularising the Cauchy problem for Laplace's equation by fractional operators

In this paper we revisit the classical Cauchy problem for Laplace's equation as well as two further related problems in the light of regularisation of this highly ill-conditioned problem by replacing integer derivatives with fractional ones. We do so in the spirit of quasi reversibility, replacing a classically severely ill-posed PDE problem by a nearby well-posed or only mildly ill-posed one. In order to be able to make use of the known stabilising effect of one-dimensional fractional derivatives of Abel type we work in a particular rectangular (in higher space dimensions cylindrical) geometry. We start with the plain Cauchy problem of reconstructing the values of a harmonic function inside this domain from its Dirichlet and Neumann trace on part of the boundary (the cylinder base) and explore three options for doing this with fractional operators. The two other related problems are the recovery of a free boundary and then this together with simultaneous recovery of the impedance function in the boundary condition. Our main technique here will be Newton's method. The paper contains numerical reconstructions and convergence results for the devised methods.

==> ell_L_fig.tex <==
%% To be added to reconstruction.tex and placed in this section.
%
\xfiglen=4 true in
\yfiglen=2.5 true in
\setbox\figuresix=\vbox{\hsize=\xfiglen 
\beginpicture
  \setcoordinatesystem units <2\xfiglen,\yfiglen>  point at 0.0 0.0
  \setplotarea x from 0.1 to 0.5, y from 0.0 to 0.9
\relax
\scriptsize
  \axis bottom ticks short numbered from 0.1 to 0.5 by 0.1 /
  \axis left ticks short numbered from 0.1 to 0.9 by 0.2 /
  %\axis left ticks short numbered from 0.02 to 0.1 by 0.02 /
\footnotesize
\put {$\|\ell-\ell_{act}\|(x)$} [l] at 0.11 0.9
\put {$\bar\ell$} [b] at 0.5 0.02
\linethickness=0.4pt
\setquadratic
\setsolid
\Black{
\plot
    0.5000    0.8252
    0.4500    0.6936
    0.4000    0.5780
    0.3500    0.4757 
    0.3000    0.3846
    0.2500    0.3031
    0.2000    0.2301
    0.1500    0.1644
    0.1000    0.1050
 /\relax}\relax
%
\endpicture
%
}

The above figure shows the $L^2$ norm reconstruction error
for various values of the rectangle aspect ratio.
Taking $L=1$, the the value of $\bar\ell$ appears as the horizontal axis
while the norm is in the vertical axis.
This shows the expected increase with increasing $\bar\ell$ but we remark
that while the increase is greater than linear it is sub-quadratic over this
range.



==> input_boxes.tex <==
\input fonts
\input pictex
\font\smallsymbol = cmmi8
\newdimen\xfiglen \newdimen\yfiglen
\newbox\figurelegendone
\newbox\figurelegendtwo
\newbox\figurelegendthree
\newbox\figureone
\newbox\figuretwo
\newbox\figurethree
\newbox\figurefour
\newbox\figurefive
\newbox\figuresix


==> introduction_sv.tex <==
\section{Introduction}

%\noteBK{Use pictures from \verb+cauchy_prob.tex+}

As its name suggests, the Cauchy Problem for Laplace's equation
% (or indeed any elliptic operator)
has a long history.

\noteBK{Add references here, e.g., \cite{Alessandrini:1997,BotchevKabanikhinShishleninTyrtyshnikov:2023}; in particular the original Hadamard ones and some of those citing Alessandrini.}

By the early-middle of the nineteenth century it was known that
prescribing the values $u$ on the boundary $\partial\Omega$
of a domain $\Omega$ where $-\triangle u = 0$ allowed $u$ to be determined
uniquely within $\Omega$ with a similar statement for ``flux'' or the value
of the normal derivative: the so-called Dirichlet and Neumann problems.
These problems held great significance for an enormous range of applications
evident at that time and provided solutions that depended continuously
on the boundary measurements.
It was also recognised that frequently a case would arise where part
of the boundary is inaccessible and no measurements could be made there.
In compensation one could measure both the value and the flux at the accessible
part: the Cauchy problem.
Since solutions of Laplace's equation can be considered as the real part
of an underlying analytic functions, the analytic continuation still allowed
uniqueness of the solution.
However, the continuous dependence on the boundary data was lost;
in fact in an extreme way.
At the beginning of the twentieth century Hadamard singled such problems
out as being ``incorrectly set'' and unworthy of mathematical study.
The backwards heat problem and the Cauchy problem were the prime exhibits.
By the middle of the century such problems had shown to have
enormous physical significance and could not be ignored from any perspective.
Methods had to be found to overcome the severe ill-conditioning.
One of the techniques suggested was the method of quasi-reversibility
of Lattes and Lions
whereby the original partial differential equation was replaced by one
in which the ``incorrect'' data allowed a well-posed recovery of its solution.
This new equation contained a parameter $\epsilon$ that allowed for
stable inversion for $\epsilon>0$ but, in addition (in a sense that had to be
carefully defined), solutions of the regularising equation converged to that
of the original as $\epsilon\to 0$.

As an example, if $\Omega$ is a rectangle with the top side inaccessible
but data can be measured on the other three sides then a basic problem
is to recover the solution $u(x,y)$ by also measuring the flux
$\frac{\partial u}{\partial y}$ at, say, the bottom edge.
In the usual language we have Dirichlet data on the two sides and Cauchy data
on the bottom.
However there is a further possibility: the top side may be a curve $\ell(x)$
and we also do not know this curve -- and want to do so.
This is a classical example of a free-boundary value problem.
A typical, and well studied, example here is of corrosion to a partly
inaccessible plate. In addition, while the original top side was, say,
a pure conductor or insulator  with either $u=0$ or
$\frac{\partial u}{\partial \nu}=0$ there,
this has now to be re-modelled as an impedance condition where the
impedance paramater is also unknown as a function of $x$.

Of course, the central issue in using quasi-reversibility
is in the choice of the regularising equation.
Here we will follow recent ideas for the backwards heat problem
and replace the usual derivative in the ``difficult'' direction
by a fractional derivative.
In the parabolic case this was a time fractional derivative and one
of the first papers taking this direction was \cite{LiuYamamoto:2010}.
It was later shown in \cite{JinRundell:2015} that the effectiveness of the
method and the choice of the fractional exponent used strongly
depended on both the final time $T$ and the frequency components in
the initial time function $u_0(x)$.
This led to the current authors proposing a multi-level version
with different fractional exponents depending on the frequencies in $u_0$,
which of course had also to appear in the measured final time and
were thus identifable, \cite{fracderiv}.
This ``split frequency'' method will also play a role in the current
problem.

However, while the use of time fractional derivatives and their behaviour
in resulting partial differential equations is now well-understood,
the same cannot be said for the case of space fractional derivatives,
see \cite{BBB}.

\medskip

\noteBK{TODO: Give more examples of applications (steelmaking?)}

Related to this are obstacle problems for elliptic problems in a domain $\Omega$
that  seek to recover an interior object $D$ from additional
boundary data comes under this classification, albeit with a
different geometry.
The boundary of $D$ can be purely conductive, or purely insulating,
or satisfy an impedance condition with a perhaps unknown parameter.
The existing literature here is again extensive.
For our purposes we wish to take advantage of the geometry described earlier
where we are able, in some sense, to separate the variables and treat each of
the differential operator's components in a distinct manner.

\medskip

\noteBK{Give overview of section contents:  (problem1, problem2, problem3)}

\textcolor{blue}{TODO}{
(unless each section is to have its own reconstruction subsection?)
\footnote{\noteBK{Yes, I think each section should have its own reconstruction subsection. The text here should probably go there}}
\medskip
In each of the problems the rectangle has different aspect ratios
 and for good reason (smile).
Perhaps keep things as is, but also give some (numerical as well as a rational)
for the dependence of the condition numbers on these ratios?
\hfill\break
This may very well be (at least slightly) different for each Problem 1:3.
\medskip
It could also be that we just declare $L=1$ in the $x$-direction??
\medskip
Remark on what (disasters) would have occured if we had taken $\ell(x)$ or
$\gamma(x)$ to be a much rougher function -- the importance of having
mostly low Fourier modes -- as per the regularisation.
I am not suggesting we try and get pictures of rough $\ell(x)$ just 
(and maybe then just maybe) give a ``number of Fourier modes that can
be recovered for a given data error.
\medskip
In Cauchy3 perhaps mention ranges that work and those that would be problematic
for the sizes of $\ell(x)$ and $\gamma(x)$
\medskip
Similar examples.
}



==> pics_Cauchy2_neum_imped_sv.tex <==
%  \PiCTeX file for BB17   Cauchy2_neum_imped
%\input colordvi
\xfiglen=4 true in
\yfiglen=2 true in
%
% \input input_boxes
%%%%%%%%%%%%%%%%%%%
%
\setbox\figurelegendtwo=\hbox{
\beginpicture
  \setcoordinatesystem units <0.06\xfiglen,0.05\yfiglen> %point at 0 -0.7
  \setplotarea x from 0 to 2, y from 0 to 6
\footnotesize
\linethickness=0.5pt
\scriptsize
   \setdashes <3pt>  \putrule from 0 3 to 1.25 3
   \setsolid
   \Black{\relax \putrule from 0 6 to 1 6 \relax}\relax
   \put {$\ell(x)$ actual}  [l] at 1.2 6
%
   \Red{\relax \putrule from 0 5 to 1 5 \relax}\relax
   \put {iter 5 } [l] at 1.2 5
%
   \Purple{\relax \putrule from 0 4 to 1 4 \relax}\relax
   \put {iter 4 } [l] at 1.2 4
%
   \Blue{\relax \putrule from 0 3 to 1 3 \relax}\relax
   \put {iter 3 } [l] at 1.2 3
%
   \Cyan{\relax \putrule from 0 2 to 1 2 \relax}\relax
   \put {iter 2 } [l] at 1.2 2
%
   \Green{\relax \putrule from 0 1 to 1 1 \relax}\relax
   \put {iter 1 } [l] at 1.2 1
%
\setdots <3pt>
   \Black{\relax \putrule from 0 0 to 1 0 \relax}\relax
   \put {$\ell(x)$ initial } [l] at 1.2 -0.1
%
\endpicture
}
%
\setbox\figuretwo=\vbox{\hsize=\xfiglen
\beginpicture
  \setcoordinatesystem units <\xfiglen,10\yfiglen>  point at 0.0 0.0
  \setplotarea x from 0 to 1, y from 0.0 to 0.1
\relax
\scriptsize
  \axis bottom ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short numbered from 0 to 0.09 by 0.01 /
  %\axis left ticks short numbered from 0.02 to 0.1 by 0.02 /
\footnotesize
%\put {\copy\figurelegendone} [rb] at 0.95 0.015
\put {$\ell(x)$} [l] at 0.02 0.1
\linethickness=0.6pt
\putrule from 1 0.0 to 1 0.1
\setdots <3pt>
\putrule from 0 0.01 to 0.66 0.01
\put {$\ell_{init}$} at 0.75 0.01
\setquadratic
\setsolid
\Black{
\plot    % actual curve
         0    0.0900
    0.0200    0.0899
    0.0400    0.0897
    0.0600    0.0893
    0.0800    0.0888
    0.1000    0.0881
    0.1200    0.0873
    0.1400    0.0864
    0.1600    0.0854
    0.1800    0.0843
    0.2000    0.0831
    0.2200    0.0819
    0.2400    0.0806
    0.2600    0.0794
    0.2800    0.0781
    0.3000    0.0769
    0.3200    0.0757
    0.3400    0.0746
    0.3600    0.0736
    0.3800    0.0727
    0.4000    0.0719
    0.4200    0.0712
    0.4400    0.0707
    0.4600    0.0703
    0.4800    0.0701
    0.5000    0.0700
    0.5200    0.0701
    0.5400    0.0703
    0.5600    0.0707
    0.5800    0.0712
    0.6000    0.0719
    0.6200    0.0727
    0.6400    0.0736
    0.6600    0.0746
    0.6800    0.0757
    0.7000    0.0769
    0.7200    0.0781
    0.7400    0.0794
    0.7600    0.0806
    0.7800    0.0819
    0.8000    0.0831
    0.8200    0.0843
    0.8400    0.0854
    0.8600    0.0864
    0.8800    0.0873
    0.9000    0.0881
    0.9200    0.0888
    0.9400    0.0893
    0.9600    0.0897
    0.9800    0.0899
    1.0000    0.0900
 /\relax}\relax
%
\linethickness=0.4pt
\setdashes <3pt>
\setsolid
\Green{\relax   % iteration 1
\plot
         0    0.0851
    0.0200    0.0849
    0.0400    0.0847
    0.0600    0.0844
    0.0800    0.0839
    0.1000    0.0834
    0.1200    0.0827
    0.1400    0.0820
    0.1600    0.0812
    0.1800    0.0804
    0.2000    0.0795
    0.2200    0.0786
    0.2400    0.0778
    0.2600    0.0769
    0.2800    0.0761
    0.3000    0.0753
    0.3200    0.0745
    0.3400    0.0738
    0.3600    0.0731
    0.3800    0.0725
    0.4000    0.0719
    0.4200    0.0714
    0.4400    0.0710
    0.4600    0.0707
    0.4800    0.0705
    0.5000    0.0704
    0.5200    0.0704
    0.5400    0.0706
    0.5600    0.0709
    0.5800    0.0713
    0.6000    0.0719
    0.6200    0.0726
    0.6400    0.0733
    0.6600    0.0742
    0.6800    0.0751
    0.7000    0.0761
    0.7200    0.0770
    0.7400    0.0780
    0.7600    0.0789
    0.7800    0.0797
    0.8000    0.0805
    0.8200    0.0811
    0.8400    0.0817
    0.8600    0.0822
    0.8800    0.0827
    0.9000    0.0830
    0.9200    0.0832
    0.9400    0.0834
    0.9600    0.0836
    0.9800    0.0836
    1.0000    0.0838
 /\relax}\relax
%
\setsolid
\Red{\relax   % iteration 2
\plot
         0    0.0851
    0.0200    0.0916
    0.0400    0.0913
    0.0600    0.0907
    0.0800    0.0899
    0.1000    0.0889
    0.1200    0.0877
    0.1400    0.0865
    0.1600    0.0853
    0.1800    0.0840
    0.2000    0.0828
    0.2200    0.0816
    0.2400    0.0804
    0.2600    0.0793
    0.2800    0.0782
    0.3000    0.0772
    0.3200    0.0763
    0.3400    0.0754
    0.3600    0.0745
    0.3800    0.0737
    0.4000    0.0730
    0.4200    0.0724
    0.4400    0.0718
    0.4600    0.0714
    0.4800    0.0711
    0.5000    0.0709
    0.5200    0.0709
    0.5400    0.0711
    0.5600    0.0715
    0.5800    0.0720
    0.6000    0.0727
    0.6200    0.0736
    0.6400    0.0746
    0.6600    0.0758
    0.6800    0.0770
    0.7000    0.0784
    0.7200    0.0797
    0.7400    0.0810
    0.7600    0.0822
    0.7800    0.0834
    0.8000    0.0844
    0.8200    0.0852
    0.8400    0.0858
    0.8600    0.0863
    0.8800    0.0867
    0.9000    0.0869
    0.9200    0.0870
    0.9400    0.0871
    0.9600    0.0871
    0.9800    0.0871
    1.0000    0.0861
 /\relax}\relax
%
\endpicture
}
%


==> pics_Cauchy3_sv.tex <==
%  \PiCTeX file for BBn
\input colordvi
\input fonts
\input pictex
\font\smallsymbol = cmmi8
\newdimen\xfiglen \newdimen\yfiglen
\xfiglen=2.7 true in
\yfiglen=2.5 true in
%
%\newbox\figurelegendone
%\newbox\figurelegendtwo
%\newbox\figurelegendthree
%\newbox\figureone
%\newbox\figuretwo
%\newbox\figurethree
%\newbox\figurefour
%\newbox\figurefive
%\newbox\figuresix
%%%%%%%%%%%%%%%%%%%
%
\setbox\figurefour=\vbox{\hsize=0.6true in
\beginpicture
  \setcoordinatesystem units <0.06\xfiglen,0.05\yfiglen> %point at 0 -0.7
  \setplotarea x from 0 to 2, y from 0 to 2
\linethickness=0.5pt
\scriptsize
   \setsolid
   \Black{\relax \putrule from 0 2 to 1 2 \relax}\relax
   \put {actual}  [l] at 1.2 2
   \Red{\relax \putrule from 0 1 to 1 1 \relax}\relax
   \put {reconstruction}  [l] at 1.2 1
\endpicture
}
%
%
\setbox\figurefive=\vbox{\hsize=\xfiglen   % values of $\ell(x)$
\beginpicture
  \setcoordinatesystem units <\xfiglen,12.0\yfiglen>  point at 0.0 0.05
  \setplotarea x from 0 to 1, y from 0.05 to 0.1
\scriptsize
  \axis bottom ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short numbered from 0.05 to 0.1 by 0.01 /
% kludge follows
\put {0.05} [r] at -0.02 0.05 \putrule from -0.01 0.05 to 0 0.05
\put {0.10} [r] at -0.02 0.1  \putrule from -0.01 0.1 to 0 0.1
% end of kludge
\footnotesize
%\put {\copy\figurelegendone} [rb] at 0.95 0.015
\put {$\ell(x)$} [l] at 0.02 0.1
\linethickness=0.6pt
%\putrule from 1 0.0 to 1 0.5
\setsolid
%\putrule from 0 0.1 to 1 0.1
%\put {$\ell_{init}$} 
\put {\copy\figurefour} [rb] at 1.0 0.055
\setquadratic
\Black{
\plot    % actual curve
         0    0.0900
    0.0200    0.0899
    0.0400    0.0897
    0.0600    0.0893
    0.0800    0.0888
    0.1000    0.0881
    0.1200    0.0873
    0.1400    0.0864
    0.1600    0.0854
    0.1800    0.0843
    0.2000    0.0831
    0.2200    0.0819
    0.2400    0.0806
    0.2600    0.0794
    0.2800    0.0781
    0.3000    0.0769
    0.3200    0.0757
    0.3400    0.0746
    0.3600    0.0736
    0.3800    0.0727
    0.4000    0.0719
    0.4200    0.0712
    0.4400    0.0707
    0.4600    0.0703
    0.4800    0.0701
    0.5000    0.0700
    0.5200    0.0701
    0.5400    0.0703
    0.5600    0.0707
    0.5800    0.0712
    0.6000    0.0719
    0.6200    0.0727
    0.6400    0.0736
    0.6600    0.0746
    0.6800    0.0757
    0.7000    0.0769
    0.7200    0.0781
    0.7400    0.0794
    0.7600    0.0806
    0.7800    0.0819
    0.8000    0.0831
    0.8200    0.0843
    0.8400    0.0854
    0.8600    0.0864
    0.8800    0.0873
    0.9000    0.0881
    0.9200    0.0888
    0.9400    0.0893
    0.9600    0.0897
    0.9800    0.0899
    1.0000    0.0900
 /\relax}\relax
%
%\linethickness=0.4pt
%\setdashes <3pt>
\setsolid
\Red{\relax   % iteration 1
\plot
         0    0.0900
    0.0200    0.0893
    0.0400    0.0887
    0.0600    0.0884
    0.0800    0.0884
    0.1000    0.0885
    0.1200    0.0886
    0.1400    0.0886
    0.1600    0.0883
    0.1800    0.0878
    0.2000    0.0869
    0.2200    0.0857
    0.2400    0.0843
    0.2600    0.0826
    0.2800    0.0808
    0.3000    0.0789
    0.3200    0.0771
    0.3400    0.0754
    0.3600    0.0738
    0.3800    0.0725
    0.4000    0.0713
    0.4200    0.0703
    0.4400    0.0696
    0.4600    0.0690
    0.4800    0.0686
    0.5000    0.0684
    0.5200    0.0683
    0.5400    0.0685
    0.5600    0.0690
    0.5800    0.0696
    0.6000    0.0703
    0.6200    0.0712
    0.6400    0.0721
    0.6600    0.0731
    0.6800    0.0740
    0.7000    0.0751
    0.7200    0.0762
    0.7400    0.0776
    0.7600    0.0794
    0.7800    0.0814
    0.8000    0.0837
    0.8200    0.0860
    0.8400    0.0882
    0.8600    0.0901
    0.8800    0.0916
    0.9000    0.0926
    0.9200    0.0932
    0.9400    0.0934
    0.9600    0.0932
    0.9800    0.0926
    1.0000    0.0900
 /\relax}\relax
%
\setsolid
\endpicture
}
%
\setbox\figuresix=\vbox{\hsize=\xfiglen  % values of $\gamma$
\beginpicture
  \setcoordinatesystem units <\xfiglen,\yfiglen>  point at 0.0 0.8
  \setplotarea x from 0 to 1, y from 0.8 to 1.4
\relax
\scriptsize
  \axis bottom ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short numbered from 0.8 to 1.4 by 0.2 /
\footnotesize
\put {$\gamma(x)$} [l] at 0.02 1.4
\linethickness=0.6pt
%\putrule from 1 0.0 to 1 0.5
%\setdots <3pt>
\setsolid
%\putrule from 0 0.1 to 0.66 0.1
\setquadratic
\Black{
\plot    % actual curve
         0    1.0000
    0.0200    1.0000
    0.0400    1.0000
    0.0600    1.0000
    0.0800    1.0000
    0.1000    1.0000
    0.1200    1.0002
    0.1400    1.0027
    0.1600    1.0127
    0.1800    1.0358
    0.2000    1.0750
    0.2200    1.1285
    0.2400    1.1891
    0.2600    1.2454
    0.2800    1.2855
    0.3000    1.3000
    0.3200    1.2855
    0.3400    1.2454
    0.3600    1.1891
    0.3800    1.1285
    0.4000    1.0750
    0.4200    1.0358
    0.4400    1.0127
    0.4600    1.0027
    0.4800    1.0002
    0.5000    1.0000
    0.5200    1.0000
    0.5400    1.0000
    0.5600    1.0000
    0.5800    1.0000
    0.6000    1.0000
    0.6200    1.0000
    0.6400    1.0000
    0.6600    1.0000
    0.6800    1.0000
    0.7000    1.0000
    0.7200    1.0000
    0.7400    1.0000
    0.7600    1.0000
    0.7800    1.0000
    0.8000    1.0000
    0.8200    1.0000
    0.8400    1.0000
    0.8600    1.0000
    0.8800    1.0000
    0.9000    1.0000
    0.9200    1.0000
    0.9400    1.0000
    0.9600    1.0000
    0.9800    1.0000
    1.0000    1.0000
 /\relax}\relax
%
\Red{\relax
\plot    % reconstructed curve
         0    1.0607
    0.0200    1.0539
    0.0400    1.0385
    0.0600    1.0167
    0.0800    0.9923
    0.1000    0.9709
    0.1200    0.9585
    0.1400    0.9603
    0.1600    0.9797
    0.1800    1.0174
    0.2000    1.0709
    0.2200    1.1351
    0.2400    1.2027
    0.2600    1.2656
    0.2800    1.3158
    0.3000    1.3464
    0.3200    1.3532
    0.3400    1.3346
    0.3600    1.2924
    0.3800    1.2311
    0.4000    1.1579
    0.4200    1.0809
    0.4400    1.0089
    0.4600    0.9493
    0.4800    0.9078
    0.5000    0.8874
    0.5200    0.8879
    0.5400    0.9064
    0.5600    0.9374
    0.5800    0.9738
    0.6000    1.0085
    0.6200    1.0351
    0.6400    1.0493
    0.6600    1.0499
    0.6800    1.0386
    0.7000    1.0196
    0.7200    0.9980
    0.7400    0.9778
    0.7600    0.9608
    0.7800    0.9469
    0.8000    0.9354
    0.8200    0.9263
    0.8400    0.9209
    0.8600    0.9209
    0.8800    0.9274
    0.9000    0.9402
    0.9200    0.9581
    0.9400    0.9793
    0.9600    1.0054
    0.9800    1.0605
    1.0000    1.2441
 /\relax}\relax
\endpicture
}


==> pics_intro.tex <==
%\input eplain
\magnification=\magstephalf
\nopagenumbers
\parindent=0pt
\baselineskip=11.5pt
\parskip=3pt
\vsize=9.5true in
\mathsurround=0.5pt
\overfullrule=0pt
\belowdisplayskip=4pt plus2pt minus 2pt
\abovedisplayskip=4pt plus2pt minus 2pt
%\input figflow
%\def\frac#1#2{{{#1}\over{#2}}}
%\input pictex
%\input fonts
%\input mssymb
%\input colordvi
%
\newdimen\xfiglen \newdimen\yfiglen
\xfiglen=2.0 true in
\yfiglen=1.75 true in
%
\newbox\textone
\newbox\texttwo
\newbox\textthree
\newbox\figureone
\newbox\figuretwo
\newbox\figurethree
\newbox\figurefour
\newbox\figurefive
%%%%%%%%%%%%%%%%%%
%%
\setbox\figureone=\vbox{\hsize=\xfiglen
\beginpicture
  \setcoordinatesystem units <\xfiglen,\yfiglen>  %point at -0.3 -1
  \setplotarea x from -0.3 to 1.3, y from -0.1 to 1.25
  \putrectangle corners at 0 0  and 1 1
\tenpoint
  \put {$\triangle u = 0$}  at 0.5 0.6
\eightpoint
  \put {Determine \Red{$\,u(x,1)$}} [b] at 0.5 1.02
  \put {$u(0,y)=0$} at 0.1 0.4
  \put {$u(1,y)=0$} at 0.9 0.4
  \put {$u(x,0) = f(x)$} [t] at 0.5 -0.02
  \put {$u_y(x,0) = g(x)$} [t] at 0.5 -0.13
\endpicture
}
%%
\setbox\figuretwo=\vbox{\hsize=\xfiglen
\beginpicture
  \setcoordinatesystem units <\xfiglen,\yfiglen> % point at
  \setplotarea x from -0.3 to 1.3, y from -0.15 to 1.3
  \putrule from 0 0  to 1 0
  \putrule from 0 0  to 0 1
  \putrule from 1 0  to 1 1
\tenpoint
  \put {$\triangle u = 0$}  at 0.5 0.6
\eightpoint
\setquadratic
 \Red{\relax
  \plot
  0 1
  0.1 0.9
  0.2 0.9
  0.3 0.95
  0.45 1
  0.55 1
  0.7 1.1
  0.8 1.1
  1 1
 / \relax}
  \put {\Red{$C$}} [br] at  0.7 1.02
  \put {$\frac{\partial u}{\partial\nu}=0$} [br] at  0.4 1.04
  \put {$\searrow$}  at  0.3 1.0
  \put {$u(0,y)=0$}  at 0.1 0.4
  \put {$u(1,y)=0$}  at 0.9 0.4
  \put {$u(x,0) = f(x)$} [t] at 0.5 -0.02
  \put {$u_y(x,0) = g(x)$} [t] at 0.5 -0.13
\endpicture
}
%%
\setbox\figurethree=\vbox{\hsize=\xfiglen
\beginpicture
  \setcoordinatesystem units <\xfiglen,\yfiglen> % point at
  \setplotarea x from -0.3 to 1.3, y from -0.2 to 1.3
  \putrule from 0 0  to 1 0
  \putrule from 0 0  to 0 1
  \putrule from 1 0  to 1 1
\tenpoint
  \put {$\triangle u = 0$}  at 0.5 0.6
\eightpoint
\setquadratic
 \Red{\relax
  \plot
  0 1
  0.1 0.9
  0.2 0.9
  0.3 0.95
  0.45 1
  0.55 1
  0.7 1.1
  0.8 1.1
  1 1
 / \relax}
  \put {\Red{$C$}} [br] at  0.7 1.02
  \put {$\frac{\partial u}{\partial\nu}+\Red{\gamma(C)}u=0$} [r] at  0.5 1.1
  \put {$\searrow$}  at  0.5 1.04
  \put {$u(0,y)=0$}  at 0.1 0.4
  \put {$u(1,y)=0$}  at 0.9 0.4
  \put {$u(x,0) = f(x)$} [t] at 0.5 -0.02
  \put {$u_y(x,0) = g(x)$} [t] at 0.5 -0.13
\endpicture
}
%%%%%%%%%%%%%%%



==> pics_inv_dirichlet.tex <==
%  \PiCTeX file for BBn
%%%%%%%%%%%%%%%%%%%
%
\setbox\figurelegendone=\hbox{
\beginpicture
  \setcoordinatesystem units <0.06\xfiglen,0.05\yfiglen> %point at 0 -0.7
  \setplotarea x from 0 to 2, y from 0 to 6
\footnotesize
\linethickness=0.5pt
\scriptsize
   \setdashes <3pt>  \putrule from 0 3 to 1.25 3
   \setsolid
   \Black{\relax \putrule from 0 6 to 1 6 \relax}\relax
   \put {$\ell(x)$ actual}  [l] at 1.2 6
%
   \Red{\relax \putrule from 0 5 to 1 5 \relax}\relax
   \put {iter 5 } [l] at 1.2 5
%
   \Purple{\relax \putrule from 0 4 to 1 4 \relax}\relax
   \put {iter 4 } [l] at 1.2 4
%
   \Blue{\relax \putrule from 0 3 to 1 3 \relax}\relax
   \put {iter 3 } [l] at 1.2 3
%
   \Cyan{\relax \putrule from 0 2 to 1 2 \relax}\relax
   \put {iter 2 } [l] at 1.2 2
%
   \Green{\relax \putrule from 0 1 to 1 1 \relax}\relax
   \put {iter 1 } [l] at 1.2 1
%
\setdots <3pt>
   \Black{\relax \putrule from 0 0 to 1 0 \relax}\relax
   \put {$\ell(x)$ initial } [l] at 1.2 -0.1
%
\endpicture
}
%
\setbox\figureone=\vbox{\hsize=\xfiglen
\beginpicture
  \setcoordinatesystem units <\xfiglen,2.0\yfiglen>  point at 0.0 0.0
  \setplotarea x from 0 to 1, y from 0.0 to 0.5
\relax
\scriptsize
  \axis bottom ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short numbered from 0 to 0.5 by 0.1 /
  %\axis left ticks numbered from 0 to 1 by 0.05 /
\footnotesize
\put {\copy\figurelegendone} [rb] at 0.95 0.015
\put {$\ell(x)$} [lb] at 0.02 0.47
\linethickness=0.6pt
\putrule from 1 0.0 to 1 0.5
\setdots <3pt>
\putrule from 0 0.1 to 0.66 0.1
%\put {$\ell_{init}$} 
\setquadratic
\Black{
\plot    % actual curve
         0    0.4500
    0.0200    0.4496
    0.0400    0.4484
    0.0600    0.4465
    0.0800    0.4438
    0.1000    0.4405
    0.1200    0.4364
    0.1400    0.4319
    0.1600    0.4268
    0.1800    0.4213
    0.2000    0.4155
    0.2200    0.4094
    0.2400    0.4031
    0.2600    0.3969
    0.2800    0.3906
    0.3000    0.3845
    0.3200    0.3787
    0.3400    0.3732
    0.3600    0.3681
    0.3800    0.3636
    0.4000    0.3595
    0.4200    0.3562
    0.4400    0.3535
    0.4600    0.3516
    0.4800    0.3504
    0.5000    0.3500
    0.5200    0.3504
    0.5400    0.3516
    0.5600    0.3535
    0.5800    0.3562
    0.6000    0.3595
    0.6200    0.3636
    0.6400    0.3681
    0.6600    0.3732
    0.6800    0.3787
    0.7000    0.3845
    0.7200    0.3906
    0.7400    0.3969
    0.7600    0.4031
    0.7800    0.4094
    0.8000    0.4155
    0.8200    0.4213
    0.8400    0.4268
    0.8600    0.4319
    0.8800    0.4364
    0.9000    0.4405
    0.9200    0.4438
    0.9400    0.4465
    0.9600    0.4484
    0.9800    0.4496
    1.0000    0.4500
 /\relax}\relax
%
\linethickness=0.4pt
\setdashes <3pt>
\setsolid
\Green{\relax   % iteration 1
\plot
         0    0.1753
    0.0200    0.1753
    0.0400    0.1753
    0.0600    0.1754
    0.0800    0.1754
    0.1000    0.1754
    0.1200    0.1754
    0.1400    0.1754
    0.1600    0.1754
    0.1800    0.1753
    0.2000    0.1752
    0.2200    0.1751
    0.2400    0.1748
    0.2600    0.1746
    0.2800    0.1743
    0.3000    0.1740
    0.3200    0.1737
    0.3400    0.1733
    0.3600    0.1730
    0.3800    0.1728
    0.4000    0.1726
    0.4200    0.1725
    0.4400    0.1725
    0.4600    0.1725
    0.4800    0.1727
    0.5000    0.1729
    0.5200    0.1731
    0.5400    0.1734
    0.5600    0.1738
    0.5800    0.1741
    0.6000    0.1743
    0.6200    0.1746
    0.6400    0.1747
    0.6600    0.1748
    0.6800    0.1749
    0.7000    0.1749
    0.7200    0.1749
    0.7400    0.1748
    0.7600    0.1748
    0.7800    0.1748
    0.8000    0.1748
    0.8200    0.1748
    0.8400    0.1749
    0.8600    0.1750
    0.8800    0.1752
    0.9000    0.1753
    0.9200    0.1755
    0.9400    0.1757
    0.9600    0.1758
    0.9800    0.1759
    1.0000    0.1759
 /\relax}\relax
%
\setsolid
\Cyan{\relax   % iteration 2
\plot
         0    0.2749
    0.0200    0.2749
    0.0400    0.2750
    0.0600    0.2752
    0.0800    0.2754
    0.1000    0.2756
    0.1200    0.2757
    0.1400    0.2757
    0.1600    0.2756
    0.1800    0.2753
    0.2000    0.2748
    0.2200    0.2741
    0.2400    0.2731
    0.2600    0.2719
    0.2800    0.2706
    0.3000    0.2691
    0.3200    0.2676
    0.3400    0.2662
    0.3600    0.2648
    0.3800    0.2637
    0.4000    0.2629
    0.4200    0.2624
    0.4400    0.2623
    0.4600    0.2625
    0.4800    0.2632
    0.5000    0.2641
    0.5200    0.2653
    0.5400    0.2667
    0.5600    0.2681
    0.5800    0.2695
    0.6000    0.2708
    0.6200    0.2718
    0.6400    0.2726
    0.6600    0.2731
    0.6800    0.2733
    0.7000    0.2733
    0.7200    0.2732
    0.7400    0.2729
    0.7600    0.2726
    0.7800    0.2725
    0.8000    0.2724
    0.8200    0.2726
    0.8400    0.2729
    0.8600    0.2735
    0.8800    0.2742
    0.9000    0.2750
    0.9200    0.2758
    0.9400    0.2767
    0.9600    0.2772
    0.9800    0.2778
    1.0000    0.2778
 /\relax}\relax
%
\setsolid
\Blue{\relax   % iteration 3
\plot
         0    0.3656
    0.0200    0.3656
    0.0400    0.3660
    0.0600    0.3664
    0.0800    0.3670
    0.1000    0.3674
    0.1200    0.3677
    0.1400    0.3676
    0.1600    0.3673
    0.1800    0.3663
    0.2000    0.3649
    0.2200    0.3627
    0.2400    0.3600
    0.2600    0.3568
    0.2800    0.3531
    0.3000    0.3491
    0.3200    0.3451
    0.3400    0.3412
    0.3600    0.3376
    0.3800    0.3346
    0.4000    0.3324
    0.4200    0.3311
    0.4400    0.3308
    0.4600    0.3314
    0.4800    0.3331
    0.5000    0.3356
    0.5200    0.3387
    0.5400    0.3422
    0.5600    0.3460
    0.5800    0.3496
    0.6000    0.3529
    0.6200    0.3557
    0.6400    0.3578
    0.6600    0.3593
    0.6800    0.3600
    0.7000    0.3602
    0.7200    0.3598
    0.7400    0.3594
    0.7600    0.3588
    0.7800    0.3585
    0.8000    0.3584
    0.8200    0.3590
    0.8400    0.3599
    0.8600    0.3616
    0.8800    0.3633
    0.9000    0.3658
    0.9200    0.3677
    0.9400    0.3702
    0.9600    0.3715
    0.9800    0.3732
    1.0000    0.3732
 /\relax}\relax
%
\setsolid
\Purple{\relax   % iteration 4
\plot
         0    0.4115
    0.0200    0.4115
    0.0400    0.4122
    0.0600    0.4126
    0.0800    0.4134
    0.1000    0.4137
    0.1200    0.4140
    0.1400    0.4135
    0.1600    0.4125
    0.1800    0.4104
    0.2000    0.4075
    0.2200    0.4034
    0.2400    0.3985
    0.2600    0.3926
    0.2800    0.3862
    0.3000    0.3792
    0.3200    0.3723
    0.3400    0.3656
    0.3600    0.3595
    0.3800    0.3544
    0.4000    0.3506
    0.4200    0.3483
    0.4400    0.3477
    0.4600    0.3487
    0.4800    0.3512
    0.5000    0.3552
    0.5200    0.3602
    0.5400    0.3660
    0.5600    0.3721
    0.5800    0.3781
    0.6000    0.3835
    0.6200    0.3884
    0.6400    0.3920
    0.6600    0.3948
    0.6800    0.3962
    0.7000    0.3971
    0.7200    0.3968
    0.7400    0.3967
    0.7600    0.3959
    0.7800    0.3961
    0.8000    0.3961
    0.8200    0.3978
    0.8400    0.3993
    0.8600    0.4028
    0.8800    0.4057
    0.9000    0.4103
    0.9200    0.4135
    0.9400    0.4179
    0.9600    0.4201
    0.9800    0.4230
    1.0000    0.4230
 /\relax}\relax
%
\setsolid
\Red{\relax   % iteration 5
\plot
         0    0.4250
    0.0200    0.4250
    0.0400    0.4258
    0.0600    0.4263
    0.0800    0.4273
    0.1000    0.4276
    0.1200    0.4277
    0.1400    0.4269
    0.1600    0.4253
    0.1800    0.4224
    0.2000    0.4184
    0.2200    0.4130
    0.2400    0.4064
    0.2600    0.3988
    0.2800    0.3904
    0.3000    0.3816
    0.3200    0.3728
    0.3400    0.3643
    0.3600    0.3568
    0.3800    0.3504
    0.4000    0.3457
    0.4200    0.3429
    0.4400    0.3421
    0.4600    0.3432
    0.4800    0.3463
    0.5000    0.3511
    0.5200    0.3572
    0.5400    0.3642
    0.5600    0.3716
    0.5800    0.3790
    0.6000    0.3858
    0.6200    0.3917
    0.6400    0.3963
    0.6600    0.3998
    0.6800    0.4017
    0.7000    0.4027
    0.7200    0.4026
    0.7400    0.4024
    0.7600    0.4016
    0.7800    0.4019
    0.8000    0.4021
    0.8200    0.4044
    0.8400    0.4067
    0.8600    0.4114
    0.8800    0.4154
    0.9000    0.4215
    0.9200    0.4259
    0.9400    0.4318
    0.9600    0.4348
    0.9800    0.4387
    1.0000    0.4387
 /\relax}\relax
%
\endpicture
}
%


==> pics_inv_dirichlet_sv.tex <==
%  \PiCTeX file for BBn
\input colordvi
\input fonts
\input pictex
\font\smallsymbol = cmmi8
\newdimen\xfiglen \newdimen\yfiglen
\xfiglen=4 true in
\yfiglen=2 true in
%
\newbox\figurelegendone
\newbox\figurelegendtwo
\newbox\figurelegendthree
\newbox\figureone
\newbox\figuretwo
\newbox\figurethree
\newbox\figurefour
\newbox\figurefive
\newbox\figuresix
%%%%%%%%%%%%%%%%%%%
%
\setbox\figurelegendone=\hbox{
\beginpicture
  \setcoordinatesystem units <0.06\xfiglen,0.05\yfiglen> %point at 0 -0.7
  \setplotarea x from 0 to 2, y from 0 to 6
\footnotesize
\linethickness=0.5pt
\scriptsize
   \setdashes <3pt>  \putrule from 0 3 to 1.25 3
   \setsolid
   \Black{\relax \putrule from 0 6 to 1 6 \relax}\relax
   \put {$\ell(x)$ actual}  [l] at 1.2 6
%
   \Red{\relax \putrule from 0 5 to 1 5 \relax}\relax
   \put {iter 5 } [l] at 1.2 5
%
   \Purple{\relax \putrule from 0 4 to 1 4 \relax}\relax
   \put {iter 4 } [l] at 1.2 4
%
   \Blue{\relax \putrule from 0 3 to 1 3 \relax}\relax
   \put {iter 3 } [l] at 1.2 3
%
   \Cyan{\relax \putrule from 0 2 to 1 2 \relax}\relax
   \put {iter 2 } [l] at 1.2 2
%
   \Green{\relax \putrule from 0 1 to 1 1 \relax}\relax
   \put {iter 1 } [l] at 1.2 1
%
\setdots <3pt>
   \Black{\relax \putrule from 0 0 to 1 0 \relax}\relax
   \put {$\ell(x)$ initial } [l] at 1.2 -0.1
%
\endpicture
}
%
\setbox\figureone=\vbox{\hsize=\xfiglen
\beginpicture
  \setcoordinatesystem units <\xfiglen,2.0\yfiglen>  point at 0.0 0.0
  \setplotarea x from 0 to 1, y from 0.0 to 0.5
\relax
\scriptsize
  \axis bottom ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short numbered from 0 to 0.5 by 0.1 /
  %\axis left ticks numbered from 0 to 1 by 0.05 /
\footnotesize
\put {\copy\figurelegendone} [rb] at 0.95 0.015
\put {$\ell(x)$} [lb] at 0.02 0.47
\linethickness=0.6pt
\putrule from 1 0.0 to 1 0.5
\setdots <3pt>
\putrule from 0 0.1 to 0.66 0.1
%\put {$\ell_{init}$} 
\setquadratic
\Black{
\plot    % actual curve
         0    0.4500
    0.0200    0.4496
    0.0400    0.4484
    0.0600    0.4465
    0.0800    0.4438
    0.1000    0.4405
    0.1200    0.4364
    0.1400    0.4319
    0.1600    0.4268
    0.1800    0.4213
    0.2000    0.4155
    0.2200    0.4094
    0.2400    0.4031
    0.2600    0.3969
    0.2800    0.3906
    0.3000    0.3845
    0.3200    0.3787
    0.3400    0.3732
    0.3600    0.3681
    0.3800    0.3636
    0.4000    0.3595
    0.4200    0.3562
    0.4400    0.3535
    0.4600    0.3516
    0.4800    0.3504
    0.5000    0.3500
    0.5200    0.3504
    0.5400    0.3516
    0.5600    0.3535
    0.5800    0.3562
    0.6000    0.3595
    0.6200    0.3636
    0.6400    0.3681
    0.6600    0.3732
    0.6800    0.3787
    0.7000    0.3845
    0.7200    0.3906
    0.7400    0.3969
    0.7600    0.4031
    0.7800    0.4094
    0.8000    0.4155
    0.8200    0.4213
    0.8400    0.4268
    0.8600    0.4319
    0.8800    0.4364
    0.9000    0.4405
    0.9200    0.4438
    0.9400    0.4465
    0.9600    0.4484
    0.9800    0.4496
    1.0000    0.4500
 /\relax}\relax
%
\linethickness=0.4pt
\setdashes <3pt>
\setsolid
\Green{\relax   % iteration 1
\plot
         0    0.1753
    0.0200    0.1753
    0.0400    0.1753
    0.0600    0.1754
    0.0800    0.1754
    0.1000    0.1754
    0.1200    0.1754
    0.1400    0.1754
    0.1600    0.1754
    0.1800    0.1753
    0.2000    0.1752
    0.2200    0.1751
    0.2400    0.1748
    0.2600    0.1746
    0.2800    0.1743
    0.3000    0.1740
    0.3200    0.1737
    0.3400    0.1733
    0.3600    0.1730
    0.3800    0.1728
    0.4000    0.1726
    0.4200    0.1725
    0.4400    0.1725
    0.4600    0.1725
    0.4800    0.1727
    0.5000    0.1729
    0.5200    0.1731
    0.5400    0.1734
    0.5600    0.1738
    0.5800    0.1741
    0.6000    0.1743
    0.6200    0.1746
    0.6400    0.1747
    0.6600    0.1748
    0.6800    0.1749
    0.7000    0.1749
    0.7200    0.1749
    0.7400    0.1748
    0.7600    0.1748
    0.7800    0.1748
    0.8000    0.1748
    0.8200    0.1748
    0.8400    0.1749
    0.8600    0.1750
    0.8800    0.1752
    0.9000    0.1753
    0.9200    0.1755
    0.9400    0.1757
    0.9600    0.1758
    0.9800    0.1759
    1.0000    0.1759
 /\relax}\relax
%
\setsolid
\Cyan{\relax   % iteration 2
\plot
         0    0.2749
    0.0200    0.2749
    0.0400    0.2750
    0.0600    0.2752
    0.0800    0.2754
    0.1000    0.2756
    0.1200    0.2757
    0.1400    0.2757
    0.1600    0.2756
    0.1800    0.2753
    0.2000    0.2748
    0.2200    0.2741
    0.2400    0.2731
    0.2600    0.2719
    0.2800    0.2706
    0.3000    0.2691
    0.3200    0.2676
    0.3400    0.2662
    0.3600    0.2648
    0.3800    0.2637
    0.4000    0.2629
    0.4200    0.2624
    0.4400    0.2623
    0.4600    0.2625
    0.4800    0.2632
    0.5000    0.2641
    0.5200    0.2653
    0.5400    0.2667
    0.5600    0.2681
    0.5800    0.2695
    0.6000    0.2708
    0.6200    0.2718
    0.6400    0.2726
    0.6600    0.2731
    0.6800    0.2733
    0.7000    0.2733
    0.7200    0.2732
    0.7400    0.2729
    0.7600    0.2726
    0.7800    0.2725
    0.8000    0.2724
    0.8200    0.2726
    0.8400    0.2729
    0.8600    0.2735
    0.8800    0.2742
    0.9000    0.2750
    0.9200    0.2758
    0.9400    0.2767
    0.9600    0.2772
    0.9800    0.2778
    1.0000    0.2778
 /\relax}\relax
%
\setsolid
\Blue{\relax   % iteration 3
\plot
         0    0.3656
    0.0200    0.3656
    0.0400    0.3660
    0.0600    0.3664
    0.0800    0.3670
    0.1000    0.3674
    0.1200    0.3677
    0.1400    0.3676
    0.1600    0.3673
    0.1800    0.3663
    0.2000    0.3649
    0.2200    0.3627
    0.2400    0.3600
    0.2600    0.3568
    0.2800    0.3531
    0.3000    0.3491
    0.3200    0.3451
    0.3400    0.3412
    0.3600    0.3376
    0.3800    0.3346
    0.4000    0.3324
    0.4200    0.3311
    0.4400    0.3308
    0.4600    0.3314
    0.4800    0.3331
    0.5000    0.3356
    0.5200    0.3387
    0.5400    0.3422
    0.5600    0.3460
    0.5800    0.3496
    0.6000    0.3529
    0.6200    0.3557
    0.6400    0.3578
    0.6600    0.3593
    0.6800    0.3600
    0.7000    0.3602
    0.7200    0.3598
    0.7400    0.3594
    0.7600    0.3588
    0.7800    0.3585
    0.8000    0.3584
    0.8200    0.3590
    0.8400    0.3599
    0.8600    0.3616
    0.8800    0.3633
    0.9000    0.3658
    0.9200    0.3677
    0.9400    0.3702
    0.9600    0.3715
    0.9800    0.3732
    1.0000    0.3732
 /\relax}\relax
%
\setsolid
\Purple{\relax   % iteration 4
\plot
         0    0.4115
    0.0200    0.4115
    0.0400    0.4122
    0.0600    0.4126
    0.0800    0.4134
    0.1000    0.4137
    0.1200    0.4140
    0.1400    0.4135
    0.1600    0.4125
    0.1800    0.4104
    0.2000    0.4075
    0.2200    0.4034
    0.2400    0.3985
    0.2600    0.3926
    0.2800    0.3862
    0.3000    0.3792
    0.3200    0.3723
    0.3400    0.3656
    0.3600    0.3595
    0.3800    0.3544
    0.4000    0.3506
    0.4200    0.3483
    0.4400    0.3477
    0.4600    0.3487
    0.4800    0.3512
    0.5000    0.3552
    0.5200    0.3602
    0.5400    0.3660
    0.5600    0.3721
    0.5800    0.3781
    0.6000    0.3835
    0.6200    0.3884
    0.6400    0.3920
    0.6600    0.3948
    0.6800    0.3962
    0.7000    0.3971
    0.7200    0.3968
    0.7400    0.3967
    0.7600    0.3959
    0.7800    0.3961
    0.8000    0.3961
    0.8200    0.3978
    0.8400    0.3993
    0.8600    0.4028
    0.8800    0.4057
    0.9000    0.4103
    0.9200    0.4135
    0.9400    0.4179
    0.9600    0.4201
    0.9800    0.4230
    1.0000    0.4230
 /\relax}\relax
%
\setsolid
\Red{\relax   % iteration 5
\plot
         0    0.4250
    0.0200    0.4250
    0.0400    0.4258
    0.0600    0.4263
    0.0800    0.4273
    0.1000    0.4276
    0.1200    0.4277
    0.1400    0.4269
    0.1600    0.4253
    0.1800    0.4224
    0.2000    0.4184
    0.2200    0.4130
    0.2400    0.4064
    0.2600    0.3988
    0.2800    0.3904
    0.3000    0.3816
    0.3200    0.3728
    0.3400    0.3643
    0.3600    0.3568
    0.3800    0.3504
    0.4000    0.3457
    0.4200    0.3429
    0.4400    0.3421
    0.4600    0.3432
    0.4800    0.3463
    0.5000    0.3511
    0.5200    0.3572
    0.5400    0.3642
    0.5600    0.3716
    0.5800    0.3790
    0.6000    0.3858
    0.6200    0.3917
    0.6400    0.3963
    0.6600    0.3998
    0.6800    0.4017
    0.7000    0.4027
    0.7200    0.4026
    0.7400    0.4024
    0.7600    0.4016
    0.7800    0.4019
    0.8000    0.4021
    0.8200    0.4044
    0.8400    0.4067
    0.8600    0.4114
    0.8800    0.4154
    0.9000    0.4215
    0.9200    0.4259
    0.9400    0.4318
    0.9600    0.4348
    0.9800    0.4387
    1.0000    0.4387
 /\relax}\relax
%
\endpicture
}
%


==> reconstructions.tex <==
\section{Reconstructions}

\textcolor{blue}{
This section was used a placeholder for all 3 problems
and has to be broken up into its components.
It also has to be expanded with corresponding text.
}

\input pics_inv_dirichlet

Figure \eqref{fig:Dirichlet} show a reconstruction of $\ell(x)$ in the case
of Dirichlet conditions
when the starting value was far from the actual curve (taken to be $y=0.1$)
and there was relatively large noise in the data.
Note the initial guess was very far from the actual curve.
No further progress in convergence took place after iteration~5.

The lateral boundary conditions were of homogeneous Neumann type

\begin{figure}[ht]
\hbox to \hsize{\hss\copy\figureone\hss\hss}
\caption{\small {\bf Recovery of $\ell(x)$ with $5\%$ noise:
$\frac{\partial u}{\partial x} = 0$ on $x=0,\ 1$,
$\ell_{\hbox{\scriptsize init}} = 0.1$
}}
\label{fig:Dirichlet}
\end{figure}
%%%%
\input pics_Cauchy2_neum_imped

Figure \eqref{fig:neum_imped} show a reconstruction of $\ell(x)$ in the case
of impedance conditions.
Note that we have taken the region in the $y-$direction to be much shorter
in this case.

The starting value was again relatively far from the actual curve
but there was now $10\%$ noise in the data.
No further progress in convergence took place after iteration~2

\begin{figure}[ht]
\hbox to \hsize{\hss\copy\figuretwo\hss\hss}
\caption{\small {\bf Recovery of $\ell(x)$ in the impedance case with
$10\%$ noise:
$\frac{\partial u}{\partial x} = 0$ on $x=0,\ 1$,
$\ell_{\hbox{\scriptsize init}} = 0.01$
}}
\label{fig:neum_imped}
\end{figure}

\bigskip
\input pics_Cauchy3
The simultaneous case of reconstructing both the curve and the impedance.
is shown in Figure~\eqref{fig:ell_and_gamma}
The starting value for the $\ell$ curve was $\ell(x) = 0.1$
and that for $\gamma$ was $\gamma(x) = 1.0$.

[more words]
 
\begin{figure}[ht]
\hbox to \hsize{\hss\copy\figurefive\hss\copy\figuresix\hss}
%
\caption{\small {\bf Simultaneous recovery of $\ell(x)$ and $\gamma(x)$}}
%The actual values are shown in black, the reconstructed in red.
\label{fig:ell_and_gamma}
\end{figure}

